Lossless 4:2:0 Screen Content Coding Using Luma-Guided Soft Context Formation

The soft context formation coder is a pixel-wise state-of-the-art lossless screen content coder using pattern matching and color palette coding in combination with arithmetic coding. It achieves excellent compression performance on screen content images in RGB 4:4:4 format with few distinct colors. In contrast to many other lossless compression methods, it codes entire color pixels at once, i.e., all color components of one pixel are coded together. Consequently, it does not natively support image formats with downsampled chroma, such as YCbCr 4:2:0, which is an often used chroma format in video compression. In this paper, we extend the soft context formation coding capabilities to 4:2:0 image compression, by successively coding Y and CbCr planes based on an analysis of normalized mutual information between image planes. Additionally, we propose an enhancement to the chroma prediction based on the luminance plane. Furthermore, we propose to transmit side-information about occurring luma-chroma combinations to improve chroma probability distribution modelling. Averaged over a large screen content image dataset, our proposed method outperforms HEVC-SCC, with HEVC-SCC needing 5.66% more bitrate compared to our method.

==> Images/lib/tikzlibrarydsp.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------
\usetikzlibrary{arrows, calc, positioning, decorations.markings}
% -------------------------------------------------------------------------
% Parameters for the library
\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block
% -------------------------------------------------------------------------
%% Define new arrow heads
%
%\pgfarrowsdeclare{dsparrow}{dsparrow}
%{
%	\arrowsize=0.25pt
%	\advance\arrowsize by .5\pgflinewidth
%	\pgfarrowsleftextend{-4\arrowsize}
%	\pgfarrowsrightextend{4\arrowsize}
%}
%{
%	\arrowsize=0.25pt
%	\advance\arrowsize by .5\pgflinewidth
%	\pgfsetdash{}{0pt} % Solid line (do not dash)
%	\pgfsetmiterjoin	 % Fixed miter join of line
%	\pgfsetbuttcap		 % Fixed butt cap of line
%	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
%	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
%	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
%	\pgfpathclose
%	\pgfusepathqfill
%}
%\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
%{
%	\arrowsize=0.25pt
%	\advance\arrowsize by .5\pgflinewidth
%	\pgfarrowsleftextend{-4\arrowsize}
%	\pgfarrowsrightextend{4\arrowsize}
%}
%{
%	\arrowsize=0.25pt
%	\advance\arrowsize by .5\pgflinewidth
%	\pgfsetdash{}{0pt}
%	\pgfsetmiterjoin
%	\pgfsetbuttcap
%	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
%	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
%	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
%	\pgfpathclose
%	\pgfusepathqfill
%}
% -------------------------------------------------------------------------
% Define new node shapes
\makeatletter
%\pgfkeys{/tikz/dsp/label/.initial=above}
% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}
%\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}
\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}
%\dspdeclareoperator{dspshapeadder}{
%	% Coordinate offset for the plus
%	\pgfutil@tempdima=\radius
%	\pgfutil@tempdima=0.55\pgfutil@tempdima
%	
%	% Draw plus
%	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
%	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
%	
%	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
%	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
%	
%	\pgfusepathqstroke
%}
%
%\dspdeclareoperator{dspshapemixer}{
%	% Coordinate offset for the cross
%	\pgfutil@tempdima=\radius
%	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
%	
%	% Draw cross
%	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
%	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
%	
%	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
%	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
%	
%	\pgfusepathqstroke
%}
%\makeatother
% -------------------------------------------------------------------------
%% Define node styles
%
%\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
%	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
%\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
%	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
%\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
%	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
%\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}
%
%% The fixed specification of text height and text depth is the somewhat
%% unaesthetic workaround to align the text in different node at the same
%% baseline. See the PGF/TikZ manual, ch. 5.1.
%\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
%	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
%\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
%	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}
%
%% -------------------------------------------------------------------------
%% Define "signal flow" lines
%
%\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
%\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
%\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
%  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}
%
%% -------------------------------------------------------------------------
%% Define various utility macros
%
%\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
%\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

